Gaussian kernel quadrature at scaled Gauss-Hermite nodes

This article derives an accurate, explicit, and numerically stable approximation to the kernel quadrature weights in one dimension and on tensor product grids when the kernel and integration measure are Gaussian. The approximation is based on use of scaled Gauss-Hermite nodes and truncation of the Mercer eigendecomposition of the Gaussian kernel. Numerical evidence indicates that both the kernel quadrature and the approximate weights at these nodes are positive. An exponential rate of convergence for functions in the reproducing kernel Hilbert space induced by the Gaussian kernel is proved under an assumption on growth of the sum of absolute values of the approximate weights.

==> plotting.tex <==
%%%%%% PLOTTING

\usepackage{tikz}
\usepackage{pgfplots}
\usepackage{color}

%% Caption packages
\usepackage[font=footnotesize,labelfont=bf]{caption}
%\usepackage{subcaption}

%% pgfplots settings
\pgfplotsset{compat=newest}
\pgfplotsset{plot coordinates/math parser=false}

% Tikz and pgfplots libraries
\usetikzlibrary{decorations.pathreplacing}
\usetikzlibrary{decorations.text}
\usetikzlibrary{patterns}
\usepgfplotslibrary{groupplots}

%% Externalize
\usetikzlibrary{external}
\tikzexternalize[
  prefix=externalized/,
  figure name=figure-ext_sec\thesection_nob 
  ]

%% Define some common lengths to be used
\newlength{\figwidth}
\setlength{\figwidth}{0.95\textwidth}
\newlength{\figheight}
\setlength{\figheight}{0.8\figwidth}

%% Some custom title commands
\newcommand{\subfigtitle}[1]{\textbf{#1}\\\vspace{0.1cm}}

%% Colors

% A bunch of different grays (larger value means lighter color)
\definecolor{gray1}{gray}{0.0}
\definecolor{gray2}{gray}{0.25}
\definecolor{gray3}{gray}{0.5}
\definecolor{gray4}{gray}{0.7}
\definecolor{gray5}{gray}{0.9}

%\colorlet{color1}{Red}
%\colorlet{color2}{BlueViolet}
%\colorlet{color3}{RawSienna}
%\colorlet{color4}{PineGreen}
%\colorlet{color5}{YellowOrange}

%\colorlet{color1}{Red}
%\colorlet{color2}{NavyBlue}
%\colorlet{color3}{Green}
%\colorlet{color4}{YellowOrange}
%\colorlet{color5}{Brown}


%\colorlet{color1}{gray1}
%\colorlet{color2}{gray2}
%\colorlet{color3}{gray3}
%\colorlet{color4}{gray4}
%\colorlet{color5}{gray5}


%% Some custom lengths

\newlength{\prel}\setlength{\prel}{0.1cm} % For pre and post offset of brackets

